Short-reach Optical Communications: A Real-world Task for Neuromorphic Hardware

Spiking neural networks (SNNs) emulated on dedicated neuromorphic accelerators promise to offer energy-efficient signal processing. However, the neuromorphic advantage over traditional algorithms still remains to be demonstrated in real-world applications. Here, we describe an intensity-modulation, direct-detection (IM/DD) task that is relevant to high-speed optical communication systems used in data centers. Compared to other machine learning-inspired benchmarks, the task offers several advantages. First, the dataset is inherently time-dependent, i.e., there is a time dimension that can be natively mapped to the dynamic evolution of SNNs. Second, small-scale SNNs can achieve the target accuracy required by technical communication standards. Third, due to the small scale and the defined target accuracy, the task facilitates the optimization for real-world aspects, such as energy efficiency, resource requirements, and system complexity.

==> discussion.tex <==
\section{Conclusion}



==> imdd_link.tex <==
\begin{tikzpicture}
        
    \node (B) at (-6.9, 1.2) {$\boldsymbol{B}$};
    \node (B) at (0, 1.2) {\input{figures/imdd.pdf_tex}};
    \node (B) at (6.9, 1.3) {$\boldsymbol{\hat{B}}$};

\end{tikzpicture}
